Topical Shifts in the Dark Web: A Longitudinal Analysis of Content from the Cybercrime Ecosystem

The dark web hosts a dynamic ecosystem of cybercrime forums and marketplaces that adapt to law enforcement pressure, technological change, and economic incentives. Prior research has extracted cyber threat intelligence from these platforms using static snapshots, with limited attention to how discussions evolve over time. In this study, we conduct a longitudinal analysis of 25,065 websites in the dark web using 11,403,638 HTML snapshots (approximately 1245.38 GB) collected over six years. We develop a longitudinal topic-modeling framework combining domain-specific embeddings, density-based clustering and temporal aggregation to measure topic prevalence and lifecycle at the website level. Our analysis identifies 55 thematic clusters. We find that approximately 75% of total discussion volume is concentrated in a small set of persistent core topics, while short-lived themes account for approximately 3% of activity. The median topic lifespan is 75 months, indicating gradual thematic evolution rather than abrupt replacement.

==> sections/0-acknowledgements.tex <==
\section*{Acknowledgement}
\noindent This work was partially supported by Hilti and the Wallenberg AI, Autonomous Systems and Software Program (WASP) funded by the Knut and Alice Wallenberg Foundation.
Part of this study is funded by the INTERSECT project, Grant No. NWA.1162.18.301, funded by NWO and by the CATRIN project, Grant No. NWA.1215.18.003. %(for RR and LA)
